KnowCoder-X: Boosting Multilingual Information Extraction via Code

Empirical evidence indicates that LLMs exhibit spontaneous cross-lingual alignment. However, although LLMs show promising cross-lingual alignment in Information Extraction (IE), a significant imbalance across languages persists, highlighting an underlying deficiency. To address this, we propose KnowCoder-X, a powerful code LLM with advanced cross-lingual and multilingual capabilities for universal IE. Firstly, it standardizes the representation of multilingual schemas using Python classes, ensuring a consistent ontology across different languages. Then, IE across languages is formulated as a unified code generation task. Secondly, we conduct IE cross-lingual alignment instruction tuning on the translated instance prediction task to enhance the model's cross-lingual transferability. During this phase, we also construct a high-quality and diverse bilingual IE parallel dataset with 257k samples, called ParallelNER, synthesized by our proposed robust three-stage pipeline, with manual annotation to ensure quality. Although without training in 29 unseen languages, KnowCoder-X surpasses ChatGPT by 30.17\% and SoTA by 20.03\%, thereby demonstrating superior cross-lingual IE capabilities. Comprehensive evaluations on 64 IE benchmarks in Chinese and English under various settings demonstrate that KnowCoder-X significantly enhances cross-lingual IE transfer through boosting the IE alignment. Our code and dataset are available at: https://github.com/ICT-GoKnow/KnowCoder

==> dataconstruct_alg.tex <==
\begin{algorithm}[t]
\caption{ IE Parallel Data Construction}

\begin{algorithmic}
    

\REQUIRE   source sentence $s^{src}$ \\ \hspace{3.27em}source entities $E^{src}$
\ENSURE target sentence $s^{tgt}$ \\
\hspace{2.62em} target entities $E^{tgt}$

\textbf{\# Generate target sentence and entities jointly.}

\STATE $s^{tgt}$, $E^{tgt}$ ← \function{Joint\_Translation($s^{src}$, $E^{src}$)} 

%\STATE \textbf{Step 2: Obtain Hard Negative Schemas}
%\STATE $Hard\_L \leftarrow \emptyset$  
\textbf{\# Find the target entities in the target sentence.}

\FOR{each $e^{src}$,$e^{tgt}$, in ($E^{src}$, $E^{tgt}$)}
    \IF{$e^{tgt}$ not in $s^{tgt}$}
        \STATE $e^{cor}$ ← \function{Find\_Entity($s^{tgt}$,$s^{src}$,$e^{src}$)}
        \IF{$e^{cor}$ in $s^{tgt}$}
            \STATE $e^{tgt}$ ← $e^{cor} $
        \ENDIF
    \ENDIF
    \ENDFOR

\textbf{\# Regenerate target sentence based on source sentence and target entities.}
\IF{not $E^{tgt}$ in $s^{tgt}$}
    \STATE $s^{tgt}$ ← \function{Regenerate($s^{src}$, $E^{tgt}$)}
\ENDIF


\end{algorithmic}
\label{alg:alg1}
\end{algorithm}

==> prompt_alignment.tex <==
\begingroup
\begin{table*}[htp]
    \centering
    %\small
    
    \begin{tabular}{p{\textwidth}}
        \toprule
        \underline{\textbf{\textsc{Instruction for Cross-Lingual Alignment.}}} \\
        \vspace{-2mm}
        \# The following is an example of Chinese Named Entity Recognition (NER) in an object-oriented programming paradigm. In this example, several entity classes are defined, and then objects of these classes are instantiated to correspond with the entities in the given sentence. \\
\\ \# Please study this example and complete the English NER task accordingly.
 \\ \\
        \# Input (Chinese NER):\\
        class Entity:\\
        
        3. Ensure the number of entities after translation matches the original number of entities.\\
        4. Output the sentence and entities separately, and ensure that the delimiter \#\#\# between the sentence and entities.\\
        5. When outputting entities, ensure only to output the translation of each entity.\\ \\
        The following is a few examples:\\ \\
        \$\{src\_lang\}\$ \{src\_key\_sentence\}: ``The EU rejected Germany's call for a boycott of British lamb.'' \#\#\# \{src\_key\_entities\}: [``EU''] \\

        \$\{tgt\_lang\}\$ \{tgt\_key\_sentence\}: ``欧盟拒绝德国呼吁抵制英国羊肉。'' \#\#\# \{tgt\_key\_entities\}: [``欧盟''] \\ \\
         \$\{src\_lang\}\$ \{src\_key\_sentence\}: ``FM involves 2 - 4.7\% of the general population with a high prevalence in women.'' \#\#\# \{src\_key\_entities\}: [] \\ 
\$\{tgt\_lang\}\$ \{tgt\_key\_sentence\}: ``FM涉及2-4.7\%的普通人口，女性中患病率较高。'' \#\#\# \{tgt\_key\_entities\}: [] \\ \\
\$\{src\_lang\}\$ \{src\_key\_sentence\}: ``Over 4000 guests from home and abroad attended the opening ceremony .'' \#\#\# \{src\_key\_entities\}: [``home'', ``Over 4000 guests from home and abroad'', ``abroad''] \\
\$\{tgt\_lang\}\$ \{tgt\_key\_sentence\}: ``超过4000名来自国内和国外的嘉宾出席了开幕式。'' \#\#\# \{tgt\_key\_entities\}: [``国内'', ``超过4000名来自国内和国外的嘉宾'', ``国外''] \\ \\

Please translate the following sentence and entities: \\ \\
\$\{src\_lang\}\$ \{src\_key\_sentence\}: ``\{src\_sentence\}'' \#\#\# \{src\_key\_entities\}: [\{entities\}] \\
\$\{tgt\_lang\}\$ \\
        \bottomrule
    \end{tabular}
    
    \caption{Prompt for Translation.}
    \label{tab:appendix-aqua-prompt}
\end{table*}
\endgroup

==> statics.tex <==
\begin{table}[htbp]
    \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{c|c|c|ccc}
    \toprule  
    \textbf{Task} & \textbf{Dataset} & \textbf{\#Type} & \textbf{\#Train} & \textbf{\#Dev} & \textbf{\#Test} \\
    \midrule
    \multirow{23}*{NER} & ACE04 & 7 & 6,202 & 745 & 812 \\
    ~ & ACE05 & 7 & 7,299 & 971 & 1,060 \\
    ~ & AnatEM & 1 & 5,861 & 2,118 & 3,830 \\
    ~ & BC2GM & 1 & 12,500 & 2,500 & 5,000 \\
    % ~ & bc4chemd & 1 & 30,682 & 30,639 & 26,364 \\
    ~ & BC5CDR & 2 & 4,560 & 4,581 & 4,797 \\
    ~ & Broad Twitter & 3 & 5,334 & 2,001 & 2,000 \\
    ~ & CoNLL 2003 & 4 & 14,041 & 3,250 & 3,453 \\
    ~ & DIANN & 1 & 3,900 & 975 & 1,334 \\
    ~ & FabNER & 12 & 9,435 & 2,182 & 2,064 \\
    ~ & FindVehicle & 21 & 21,565 & 20,777 & 20,777 \\
    ~ & GENIA & 5 & 15,023 & 1,669 & 1,854 \\
    % ~ & HarveyNER & 4 & 3,967 & 1,301 & 1,303 \\
    ~ & MIT Movie & 12 & 9,774 & 2,442 & 2,442 \\
    ~ & MIT Restaurant & 8 & 7,659 & 1,520 & 1,520 \\
    ~ & MultiNERD & 16 & 134,144 & 10,000 & 10,000 \\
    ~ & ncbi-disease & 1 & 5,432 & 923 & 940 \\
    % ~ & Ontonotes & 18 & 59,924 & 8,528 & 8,262 \\
    ~ & Ontonotes 5 & 18 & 107,032 & 14,110 & 10,838 \\
    % ~ & Polyglot-NER & 3 & 393,982 & 10,000 & 10,000 \\
    % ~ & TweetNER7 & 7 & 7,111 & 886 & 576 \\
    ~ & WikiANN & 3 & 20,000 & 10,000 & 10,000 \\
    % ~ & WikiNeural & 3 & 92,720 & 11,590 & 11,597 \\
    ~ & WNUT17 & 6 & 3,394 & 1,008 & 1,287 \\
    ~ & CrossNER\_AI & 13 & 100 & 350 & 431 \\
    ~ & CrossNER\_Literature & 11 & 100 & 400 & 416 \\
    ~ & CrossNER\_Music & 12 & 100 & 380 & 465 \\
    ~ & CrossNER\_Politics & 8 & 199 & 540 & 650 \\
    ~ & CrossNER\_Science & 16 & 200 & 450 & 543 \\
    \midrule
    \multirow{8}*{RE} & ACE05 & 6 & 10,051 & 2,420 & 2,050 \\
    ~ & ADE corpus & 1 & 3,417 & 427 & 428 \\
    ~ & CoNLL 2004 & 5 & 922 & 231 & 288 \\
    ~ & GIDS & 4 & 8,526 & 1,417 & 4,307 \\
    ~ & kbp37 & 18 & 15,917 & 1,724 & 3,405 \\
    ~ & NYT & 24 & 56,196 & 5,000 & 5,000 \\
    % ~ & NYT11 & 12 & 62,648 & 149 & 369 \\
    ~ & SciERC & 7 & 1,861 & 275 & 551 \\
    ~ & semeval RE & 10 & 6,507 & 1,493 & 2,717 \\
    \midrule
    \multirow{2}*{EE} & ACE05 & 33 & 19,216 & 901 & 676 \\
    ~ & CASIE & 5 & 11,189 & 1,778 & 3,208 \\
    \bottomrule
    \end{tabular}
    }
    \caption{\label{sft2-stat}
Statistics of the specific domain of English IE.}
\end{table}
